Construction of Molecular Dynamics Like Cellular Automata Models for Simulation of Compressible Fluid Dynamic Systems

This study aims at finding a method for constructing molecular dynamics like models using the formalism of cellular automata for fast simulation of fluid dynamic systems (including compressible phenomena). In as much as the results indicate, the attempt is successful. A systematic method for constructing cellular automata models of fluid dynamic systems is discovered and proposed following a review of the existing developments. The considerations required for constructing such models for fluid dynamic systems consisting of particles with arbitrary interaction potentials and existing over arbitrary spatial lattices are outlined. The method is illustrated by constructing a model for simulation of systems of particles moving with unit speed along the links of an underlying square spatial lattice. Using this model, two two-dimensional systems are simulated and studied for a number of model and system parameters. For almost all the model and system parameters, the results are found to be in complete agreement with the available theoretical predictions. For some model parameters, results show (expected) departure from theoretical predictions which is explained.

==> chap0/ack.tex <==
\acknowledgements

\dialogue{\em \ldots chukle chukle chukle \ldots\\
	  Verbalize.\\
	  \em Who comes first?\\
	  \ldots\ ?!\\
	  \em The one who plants or the one who nurtures.\\
	  \ldots!\\
	  \em Ah! Naturally. \ldots}

\first The support required for completion of this work was provided
by Dr.\ E.\ Rathakrishnan, my thesis supervisor. Had he not given me
an unusual freedom---to choose my path and my tools as if I knew the
destination and the terrain to cross, to roam around as if I were lost
among tall mountains, to drink innumerable cups of tea as if there
were no other edibles, to embrace fire as if it were the essence of
life, and to sleep for unusually long hours or not to sleep at all as
if I had serious work to do in both the worlds---this work would never
even have been undertaken, what to say of its conclusion. He has been
the driving force behind this work---supporting at all strange and
critical bends, inspiring, renewing confidence, and invigorating me
with energy again and again without as much as a single question. He
is an extremely demanding yet freedom loving man who knows its meaning
and knows that others need it too, a man of faith who knows that it
works wonders and can be held in place only with threads of
unquestioning honesty reaching from end to end. Dr.\ E.\ Rathakrishnan
has been a most observant, extremely patient, and careful thesis
supervisor.

I was introduced to cellular automata in the context of image
processing in a course in electrical engineering taught by Dr.\ E.\
G.\ Rajan. And a peculiar turn that my thought took also occurred in
that course when he asked me to model gas dynamics using cellular
automata, as a full semester assignment problem. It was a tough job,
but I did not know that and took it up. Knowing fully well the
difficulties and the implications of success, he was constantly
vigilant and helped me at every point in all possible ways that he
could find. He left the institute after the course was over, giving me
an ``A'' grade. He did not seem to think that I had achieved much and
also did not know that he had changed my entire thought process. As a
consequence of the course and the assignment problem, I had developed
a way of looking at things in which the entire world was discrete. In
the next semester, during the literature survey, I was convinced that
nothing but microscopic approach will give me what I want; only if
molecular dynamics can be made faster. I {\em knew\/} it can be done
using cellular automata, but ``How?'' was the problem. Dr.\ E.\ G.\
Rajan is the one who implanted the seeds for this work in my mind
which fructified after fifteen thousand cups of tea, twenty five
thousand cigarettes and thousands of sleepless nights.

During this work I had to expand my field of knowledge from gas
dynamics to computer science, discrete mathematics, and physics
(particularly theories of space-time, complex systems, interparticle
interactions, and many body problems). During this process I feel
fortunate to have held enlightening discussions with Deepak Murthy and
Jitendra Das on issues related to many aspects of computing, computer
science, formal systems, and computer architecture. Discussions with
Venu Gopal Rao, a man of great experience and expertise, on
computational methods, particularly finite element method, have found
their place in this work in the form of certain abstractions.

Lengthy and indepth discussions with P.\ V.\ K.\ Reddy and Shreesh
Jadhav on various aspects of human life, particularly society,
history, philosophy, religion, and psychology were the major factors
in my unlocking of ideas. Without them, perhaps, I would never express
myself in the way I do now.

I am convinced that nobody, other than the lab mates and coworkers,
can understand the problems and frustrations of a research scholar and
give appropriate support when needed. The company of T.\ J.\ Ignatius,
S.\ Elangovan, K.\ Srinivasan, Rahul Konnur, Bhadri Srinivas, Sujay
Datta, Shanti Lal Das, Alok Sharan, Alok Srivastava, Shashi Bhushan
Verma, Kumar Neeraj Sachdev, Manish Shreekhande, G.\ K.\ Singh,
Sirshendu De, Subir Bhattacharjee, Swapan Chakraborty, Raghunath
Behera, Dipak Sathpati, Rajesh Khanna, Brijesh Pandey, and Sudipto
Ghosh had been very pleasant and supportive through out this work.

It is hard to accept that ideas can be generated while teaching even
in a brain that is almost always clogged with them. I experienced it,
and had to accept, while explaining the Kac master kinetic equation,
workings and philosophy of the direct simulation Monte-Carlo method,
and their interrelationship to V.\ Manoj Kumar while he was working on
his Masters' dissertation with my supervisor. The insight gained from
monologues delivered to him turned out to be very useful in the
investigations presented herein.

The help given by Suresh Mishra, Sharad Chauhan, and S.\ S.\ Chauhan
simplified some administrative jobs and saved many days of precious
time. The computer center staff and system engineers, particularly
Aftab Alam and Nirmal Roberts, have been very helpful continuously.
Through A.\ K.\ P.\ Rajpal, a very practical man with great knowledge
and experience in construction and working of electronic devices, I
came to know of a number of shortcomings in the attitude of typical
scientists and novices aiming to be scientists and pitfalls in their
scientific career.

\comment{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
I also wish to acknowledge all those who made contacts as friends,
though only to make their ends meet. I am deeply indebted to them for
some of the most important and some of the most bitter experiences of
my life, none of which I can forget.

Had it not been for the overwhelming amount of mental energy which
they spent in analyzing me, I would have never come to know about
myself and, of course, much time would have been saved.

this work would have taken a few semesters less for its completion.

Finally, I wish to acknowledge the {\em anonymous\/} referee's of {\em
Physical Reviews\/} and {\em Europhysics Letters\/} for without their
remarks I would never have understood in the same depth, as I possess
now, the meaning and objectives of science and scientific research
that are upheld by many. And not to mention that without them this
work would never have taken its present form and would have got
completed two years earlier.

That scientists and engineers can be good philosophers and writers has
been taken to be a myth since long. Perhaps it was this impression
that made those who saw the drafts of this dissertation ask for the
source of dialogues written at the head of each chapter and refuse to
believe with explicit contempt that there was no reference. This
attitude, though unacceptably negative, finally turned out to be high
compliment. The dialogues are bits of deeply felt emotions and
philosophy which have managed to break loose from the subconscious
during long, lonely, and peaceful night walks and got imprinted on
paper in the same sequence of development as the chapters of this
dissertation. 

This reaction showed without ambiguity that I have surpassed the
expectations of those around me, and turned out to be an enthralling
regard for me. The dialogues have been written by myself. They are
bits of deeply felt emotions and philosophy which have managed to
break loose during long, lonely, and peaceful night walks from the
subconscious and get imprinted on paper in the same sequence of
development as the chapters of this dissertation.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vskip2\baselineskip

\null\hfill\authordate


==> chap0/dedic.tex <==
\dedication

\null
\vfill

\centerline{\LARGE\raisebox{1em}{\psl To }
            \pbf Mom, Dad, Swati, Udit, and Madhuri}

\vfill
\null
\vfill
\null


==> chap0/syn.tex <==
\chapter*{Synopsis}
\addcontentsline{toc}{chapter}{\protect\numberline {}Synopsis}

\first This study aims at finding a method for constructing molecular
dynamics like models using the formalism of cellular automata for fast
simulation of fluid dynamic systems (including compressible
phenomena). In as much as the results indicate, the attempt is
successful. A systematic method for constructing cellular automata
models of fluid dynamic systems is discovered and proposed following a
review of the existing developments. The considerations required for
constructing such models for fluid dynamic systems consisting of
particles with arbitrary interaction potentials and existing over
arbitrary spatial lattices are outlined. The method is illustrated by
constructing a model for simulation of systems of particles moving
with unit speed along the links of an underlying square spatial
lattice. Using this model, two two-dimensional systems are simulated
and studied for a number of model and system parameters. For almost
all the model and system parameters, the results are found to be in
complete agreement with the available theoretical predictions. For
some model parameters, results show (expected) departure from
theoretical predictions which is explained. The layout, contents, and
major findings of various chapters are as described below.

\paragraph{Chapter \ref{Chap:Intro}:}

Broad overview of the scope of fluid dynamics, general aspects of
modeling, and modeling of fluid dynamic systems using conventional
calculus based approach is presented. Distinction is established
between {\em computational models\/} and {\em computational
methods\/}. Difficulties in modeling and computer simulation of fluid
dynamic systems using existing calculus based models are discussed.
Use of a formalism other than calculus for modeling of fluid dynamic
systems is found to be the only remedy for difficulties encountered in
study of fluid dynamic systems using calculus based models. Cellular
automata are proposed as plausible alternate formalism for developing
microscopic models of fluid dynamic systems which, besides being
insusceptible to the problems encountered in using conventional
calculus based models, are computer friendly and computationally fast.
The broad and the exact objectives of the present investigation are
outlined. The exact objective being {\em ``to find a method for
constructing molecular dynamics or molecular dynamics like models
using cellular automata for simulation of compressible fluid dynamic
systems''\/}.

\paragraph{Chapter \ref{Chap:CALG}:}

Broad overview of the formalism of cellular automata is presented.
Wolfram's conception of cellular automata as fully discrete abstract
mathematical systems \cite{Wolfram86book,Wolfram84PDa} and the basic
elements of cellular automata, {\em viz.\/}, lattice of sites,
evolution axis, lattice sites values, evolution neighborhood, and
evolution rules are described. It is found that basic elements of
cellular automata, owing to their abstraction, can be interpreted in
many different ways for modeling of physical systems and thus, many
different types of models can be developed. The existing cellular
automata models of physical systems, known as {\em lattice gases\/},
are renamed as {\em ``multiparticle lattice gases''\/} because in them
lattice sites values are interpreted as representing the state of more
than one particle. Growth of multiparticle lattice gases starting from
origin of the concept in 1963 \cite{Huang63book} till most recent
({\em i.e.\/}, till 1997) and multifarious developments in modeling,
simulation, and analysis ({\em e.g.\/}, \cite{Boghosianetal97}) are
reviewed. Different representations of multiparticle lattice gases,
{\em viz.\/}, {\em partitioned spatial lattice representation\/} and
{\em multiple particle representation\/}, are outlined. Some
multiparticle lattice gases of interest in the present investigation,
{\em viz.\/}, HPP gas \cite{Hardyetal73,Hardyetal76}, BBMCA model
\cite{Margolus84,Toffolietal87book}, TM gas \cite{Toffolietal87book},
and FHP gas \cite{Frischetal86,Wolfram86,Frischetal87CS}, are
described. Generalized definition of multiparticle lattice gases and
major steps involved in their mathematical analysis which leads to
various kinetic and hydrodynamic equations are outlined. Some problems
with multiparticle lattice gases, {\em viz.\/}, violation of Galilean
invariance and incorrect simulation of compressible systems and
phenomena, and their causes explained in the literature are critically
reviewed. Arguments contesting the validity and completeness of these
explanations are presented. It is found that if these problems can be
overcome, multiparticle lattice gases would make good molecular
dynamics like cellular automata models of physical systems. Finally,
it is concluded that problems encountered with multiparticle lattice
gases need to be analyzed afresh.

\paragraph{Chapter \ref{Chap:CauseProbs}:}

The conceptual representations of multiparticle lattice gases are
analyzed. The partitioned spatial lattice representation, although
computationally efficient, is found to be physically inconsistent. The
multiple particle representation is found to be correct and physically
consistent representation for multiparticle lattice gases. The twin
problems with multiparticle lattice gases are rigorously analyzed
afresh. It is observed that nonlinear terms of the momentum
(Navier-Stokes) equation encode the mechanism of spatial momentum
redistribution in physical systems. In physical systems two different
microscopic processes, {\em viz.\/}, translation of particles and
interparticle interactions, cause redistribution of momentum in space
\cite{Chapmanetal70book}. Thus, nonlinear terms of the momentum
equation encode, and originate from, the combined effect of these two
microscopic mechanisms of spatial momentum redistribution. In
multiparticle lattice gases interactions occur among particles
occupying the same lattice site (by definition). As a result, in them
particles behave like {\em rigid point particles\/} and spatial
momentum redistribution does not occur during interparticle
interactions. In view of this, it is concluded that in multiparticle
lattice gases violation of Galilean invariance and incorrect
simulation of compressible phenomena occur because of lack of spatial
momentum redistribution during interparticle interactions. Since
interparticle interactions are encoded into collision rules of
multiparticle lattice gases, it is also concluded that the structure
of collision rules plays key role in the macroscopic dynamics of
multiparticle lattice gases.

\paragraph{Chapter \ref{Chap:OverProbs}:}

Requirements and methods of overcoming the problems with multiparticle
lattice gases are discussed and whether or not these lattice gases can
be improved is analyzed. Restoring spatial momentum redistribution
during interparticle interactions is found to be necessary for
overcoming the problems. This can be done by incorporating a mechanism
into lattice gases so that interactions occur among particles
occupying different lattice sites. This condition, although necessary,
is insufficient by itself. Analysis shows that the problems can be
overcome by allowing at most one or zero particle to occupy a lattice
site at any time step (necessary and sufficient condition). This
constraint is termed as {\em ``single particle exclusion
principle''\/}. It is found that this exclusion principle cannot be
incorporated into multiparticle lattice gases without altering their
basic definition and structure; which makes the resulting lattice
gases very different from multiparticle lattice gases. In view of this
it is concluded that the twin problems cannot be removed from
multiparticle lattice gases. The lattice gases based on this exclusion
principle are termed as {\em ``single particle lattice gases''\/}.
Consequences of the single particle exclusion principle, {\em e.g.\/},
being able to associate desired interaction potentials with particles,
are discussed. It is found and concluded that single particle lattice
gases are the desired fully discrete analogs of molecular dynamics.

\paragraph{Chapter \ref{Chap:ConsSPLG}:}

The considerations which are necessary for constructing single
particle lattice gases, {\em viz.\/}, considerations related to length
scales, time scales, interaction potential, range of interactions,
types of interparticle interactions, interaction neighborhoods,
discrete velocity sets, and determination of time step $\Delta t$ and
lattice parameters of single particle lattice gases in terms of
corresponding physical parameters, are outlined. It is found that for
simulation of fluid dynamic systems single particle lattice gases can
be constructed under the following assumptions: (i) at any time step
particles undergo zero or one collision with one or many neighbors,
and (ii) $\Delta t_{\rm C} \ll \Delta t$, where $\Delta t_{\rm C}$ is
collision time. These assumptions are equivalent to the first basic
assumption in Boltzmann's analysis of gases, {\em viz.\/}, $\Delta
t_{\rm C} \ll t_{\rm mft}$, where $t_{\rm mft}$ is the mean free time
or the relaxation time \cite{Chapmanetal70book,Wu66book}. Generalized
definition of single particle lattice gases, including generalized
description of evolution strategy wherein evolution during each time
step is decomposed into two sequential sub-steps, {\em viz.\/}, (i)
processing of interparticle interactions, and then (ii) processing of
particle translation, are presented. This decomposition is equivalent
to decomposing the evolution operator ${\cal E}$ of the system into
interaction operator ${\cal C}$ and translation operator ${\cal T}$ as
${\cal E} = {\cal T}{\cal C}$. The operators ${\cal T}$ and ${\cal C}$
are, in general, non-commutative. This is in contrast with
multiparticle lattice gases.

It is found that due to single particle exclusion principle a new type
of global coupling arises among particles in single particle lattice
gases despite the fact that all interparticle interactions are local.
This global coupling is termed as {\em ``exclusion global
coupling''\/}. This global coupling cannot be eliminated and
necessitates that the interaction rules be developed by considering
the entire spatial lattice as interaction neighborhood of particles.
This being infeasible, in turn, necessitates that overall interaction
operator ${\cal C}$ be expanded recursively in terms of fractional
interaction operator ${\cal C}'$ as
\[
  {\cal C} = \underbrace{{\cal C}' {\cal C}' \cdots {\cal C}'}_{{\cal
  N}_{\rm iter}}
\]
where ${\cal N}_{\rm iter}$ is total number of terms in the expansion
and ${\cal C}'$ is constructed over a small (compared to the spatial
lattice) interaction neighborhood. This recursive decomposition makes
the processing of interparticle interaction an iterative process. The
operators ${\cal C}$ and ${\cal C}'$, in general, contain
probabilistic elements; which inhibits {\em a priori\/} determination
of ${\cal N}_{\rm iter}$. Finally, the generalized method of
construction of fractional interaction rules is described.

\paragraph{Chapter \ref{Chap:SPLG-1}:}

A two-dimensional single speed single species single particle lattice
gas existing over square spatial lattice is constructed for
demonstrating the method outlined in chapter~\ref{Chap:ConsSPLG}. Some
aspects of mathematical analysis of this lattice gas are presented.
This lattice gas is termed as {\em ``SPLG-1''\/} model or {\em
``SPLGA-1''\/} model for identification in the following chapters. The
acronym SPLG(A) stands for {\bf S}ingle {\bf P}article {\bf L}attice
{\bf G}as ({\bf A}utomata).

\paragraph{Chapter \ref{Chap:Sim1}:}

Results of simulation of two-dimensional system of particles enclosed
in a box at equilibrium carried out using the SPLG-1 model for five
different model parameters and two different densities are presented.
Mean displacement and mean square displacement (second integral of
velocity autocorrelation function) of tagged particles and time
correlation function for velocity at lattice sites are sampled.
Correlation function is found to decay as $t^{-1}$ at long times.
Other results agree with predictions of the Langevin equation.
Departure, where ever seen, is explained and found to be controllable
feature of the model.

\paragraph{Chapter \ref{Chap:Sim2}:}

Results of simulation of relaxation of strong density perturbation in
finite length two-dimensional tube carried out using the SPLG-1 model
are presented. Mean density and mean $x$- and $y$-momentum are sampled
along the centerline of the tube. Observed dynamics of formation,
propagation, and reflection (from a solid wall) of density and
momentum waves in the tube is analyzed. The results are first of their
kind in the literature and no rigorous comparison is feasible. The
profile of the leading edge of density wave, however, is compared with
existing theoretical results for other systems and both are found to
be similar.

\paragraph{Chapter \ref{Chap:Conc}:}

Achievements, failures, and difficulties encountered during the study
are summarized. The major conclusions are: (i) it is indeed possible
to develop molecular dynamics like models for simulation of fluid
dynamic systems using cellular automata, and (ii) a systematic and
algorithmic method has been discovered for constructing such models.

\paragraph{Chapter \ref{Chap:ScopeNDir}:}

Some plausible offshoots and extensions of this study are pointed out
and directions for further work along similar lines are given.

\null

%\bibliographystyle{Tunsrt}
%\input{ALLBIB}
\input{chap0.bbl}


==> chap2/T2N1RCA.tex <==
\begin{tabular}{@{}|c|c||cccc|@{}}
\hline
  \begin{tabular}{@{}c@{}}
    Input \\
    state \\
  \end{tabular} &
    \begin{tabular}{@{}c@{}}
      Input \\
      states \\
    \end{tabular} &
      \multicolumn{4}{c|@{}}{\begin{tabular}{@{}c@{}}
			       Output states for \\
			       evolution rule number \\
			     \end{tabular}} \\
\cline{3-6}
  number &
    &
      \makebox[5mm]{0} &
        \makebox[5mm]{1} &
	  \makebox[5mm]{2} &
	    \makebox[5mm]{3} \\
\hline\hline
   0 &
     $\circ$   &
       $\circ$   &
	 $\bullet$ &
	   $\circ$   &
	     $\bullet$ \\
   1 &
     $\bullet$ &
       $\circ$   &
         $\circ$   &
	   $\bullet$ &
	     $\bullet$ \\
\hline
\end{tabular}


==> chap2/T2N2RCA.tex <==
\begin{tabular}{@{}|c|cc||cccccccccccccccc|@{}}
\hline
  \begin{tabular}{@{}c@{}}
    Input \\
    state \\
  \end{tabular} &
    \multicolumn{2}{c||}{\begin{tabular}{@{}c@{}}
			   Input \\
			   states \\
			 \end{tabular}} &
      \multicolumn{16}{c|@{}}{Output states for evolution
                              rule number} \\
\cline{4-19}
  number & & &
     0 &
       1 &
	 2 &
	   3 &
	     4 &
	       5 &
		 6 &
		   7 &
		     8 &
		       9 &
			 10 &
			   11 &
			     12 &
			       13 &
				 14 &
				   15 \\
\hline\hline
   0 & $\circ$   & $\circ$   &
     $\circ$ &
       $\bullet$ &
	 $\circ$ &
	   $\bullet$ &
	     $\circ$ &
	       $\bullet$ &
		 $\circ$ &
		   $\bullet$ &
		     $\circ$ &
		       $\bullet$ &
			 $\circ$ &
			   $\bullet$ &
			     $\circ$ &
			       $\bullet$ &
				 $\circ$ &
				   $\bullet$ \\
   1 & $\circ$   & $\bullet$ &
     $\circ$ &
       $\circ$ &
	 $\bullet$ &
	   $\bullet$ &
	     $\circ$ &
	       $\circ$ &
		 $\bullet$ &
		   $\bullet$ &
		     $\circ$ &
		       $\circ$ &
			 $\bullet$ &
			   $\bullet$ &
			     $\circ$ &
			       $\circ$ &
				 $\bullet$ &
				   $\bullet$ \\
   2 & $\bullet$ & $\circ$   &
     $\circ$ &
       $\circ$ &
	 $\circ$ &
	   $\circ$ &
	     $\bullet$ &
	       $\bullet$ &
		 $\bullet$ &
		   $\bullet$ &
		     $\circ$ &
		       $\circ$ &
			 $\circ$ &
			   $\circ$ &
			     $\bullet$ &
			       $\bullet$ &
				 $\bullet$ &
				   $\bullet$ \\
   3 & $\bullet$ & $\bullet$ &
     $\circ$ &
       $\circ$ &
	 $\circ$ &
	   $\circ$ &
	     $\circ$ &
	       $\circ$ &
		 $\circ$ &
		   $\circ$ &
		     $\bullet$ &
		       $\bullet$ &
			 $\bullet$ &
			   $\bullet$ &
			     $\bullet$ &
			       $\bullet$ &
				 $\bullet$ &
				   $\bullet$ \\
\hline
\end{tabular}


==> chap2/T3N1RCA.tex <==
\begin{tabular}{@{}|c|c||cccccccccccccc|@{}}
\hline
  \begin{tabular}{@{}c@{}}
    Input \\
    state \\
  \end{tabular} &
    \begin{tabular}{@{}c@{}}
      Input \\
      states \\
    \end{tabular} &
      \multicolumn{14}{c|@{}}{Output states for evolution
                              rule number} \\
\cline{3-16}
  number & &
     0 &
       1 &
	 2 &
	   3 &
	     4 &
	       5 &
		 6 &
		   7 &
		     8 &
		       9 &
			 10 &
			   11 &
			     12 &
			       13 \\
\hline\hline
   0 & $\circ$ &
     $\circ$ &
       $\bullet$ &
	 $\star$ &
	   $\circ$ &
	     $\bullet$ &
	       $\star$ &
		 $\circ$ &
		   $\bullet$ &
		     $\star$ &
		       $\circ$ &
			 $\bullet$ &
			   $\star$ &
			     $\circ$ &
			       $\bullet$ \\
   1 & $\bullet$ &
     $\circ$ &
       $\circ$ &
	 $\circ$ &
	   $\bullet$ &
	     $\bullet$ &
	       $\bullet$ &
		 $\star$ &
		   $\star$ &
		     $\star$ &
		       $\circ$ &
			 $\circ$ &
			   $\circ$ &
			     $\bullet$ &
			       $\bullet$ \\
   2 & $\star$ &
     $\circ$ &
       $\circ$ &
	 $\circ$ &
	   $\circ$ &
	     $\circ$ &
	       $\circ$ &
		 $\circ$ &
		   $\circ$ &
		     $\circ$ &
		       $\bullet$ &
			 $\bullet$ &
			   $\bullet$ &
			     $\bullet$ &
			       $\bullet$ \\
\hline
\multicolumn{16}{@{}c@{}}{}\\
\hline
  \begin{tabular}{@{}c@{}}
    Input \\
    state \\
  \end{tabular} &
    \begin{tabular}{@{}c@{}}
      Input \\
      states \\
    \end{tabular} &
      \multicolumn{14}{c|@{}}{Output states for evolution
                              rule number} \\
\cline{3-16}
  number & &
     14 &
       15 &
	 16 &
	   17 &
	     18 &
	       19 &
		 20 &
		   21 &
		     22 &
		       23 &
			 24 &
			   25 &
			     26 & \\
\hline\hline
   0 & $\circ$ &
     $\star$ &
       $\circ$ &
	 $\bullet$ &
	   $\star$ &
	     $\circ$ &
	       $\bullet$ &
		 $\star$ &
		   $\circ$ &
		     $\bullet$ &
		       $\star$ &
			 $\circ$ &
			   $\bullet$ &
			     $\star$ & \\
   1 & $\bullet$ &
     $\bullet$ &
       $\star$ &
	 $\star$ &
	   $\star$ &
	     $\circ$ &
	       $\circ$ &
		 $\circ$ &
		   $\bullet$ &
		     $\bullet$ &
		       $\bullet$ &
			 $\star$ &
			   $\star$ &
			     $\star$ & \\
   2 & $\star$ &
     $\bullet$ &
       $\bullet$ &
	 $\bullet$ &
	   $\bullet$ &
	     $\star$ &
	       $\star$ &
		 $\star$ &
		   $\star$ &
		     $\star$ &
		       $\star$ &
			 $\star$ &
			   $\star$ &
			     $\star$ & \\
\hline
\end{tabular}


==> chap2/TCANot.tex <==
\begin{tabular}{@{}|l|p{0.8\textwidth}|@{}}
\hline
Symbol                & Meaning\slash representation \\
\hline\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
${\cal D}$            & Dimensionality of the spatial lattice of sites
			or cells. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\{i\}$               & Coordinate of a lattice site in ${\cal
			D}$-dimensional space. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$t$                   & Time step. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
${\cal A}$            & Discrete value (or, symbol) set. It,
			necessarily, contains finitely many elements
			(values or symbols). \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$A_{\{i\}}^{(t)}$     & Value of lattice site $\{i\}$ at time step
                        $t$. $A_{\{i\}}^{(t)} \in {\cal A}$.
			\\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\{A_{\{i\}}\}$       & Values of lattice sites in the spatial
			neighborhood of lattice site $\{i\}$.
			Spatial neighborhood necessarily contains
			finitely many lattice sites. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\left\{A_{\{i\}}^{(t)}\right\}$ &
                        Values of lattice sites in the spatial
			neighborhood of lattice site $\{i\}$ at
			time step $t$.
			Spatial neighborhood necessarily contains
			finitely many lattice sites. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\tau$                & Number of preceding time steps on which the
                        new value ({\em i.e.\/}, value at time step
			$t+1$) of lattice site $\{i\}$ depends.
			$\tau$ is necessarily finite and
			$\tau = 1, 2, 3, \ldots$. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\left\{A_{\{i\}}^{(t)}\right\}^{(\tau)}$ &
                        Values of lattice sites in the spatio-temporal
			neighborhood of lattice site $\{i\}$.
			The temporal neighborhood extends to $\tau$
			preceding time steps, {\em i.e.\/}, from time
			step $\tau$ to time step $t-\tau+1$.
			Spatial neighborhood at each time step
			necessarily contains finitely many lattice
			sites and different preceding time steps can,
			in general, be different.
			If $\tau = 1$, the superscript $(\tau)$ is
			omitted. Thus, \newline
\centerline{$
  \left\{A_{\{i\}}^{(t)}\right\}^{(1)} \equiv
  \left\{A_{\{i\}}^{(t)}\right\}
$}
			\\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\Gamma^{(t)}$        & State of the entire system, {\em i.e.\/}, all
			the lattice sites comprising the system, at
			time step $t$. \\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\left\{\Gamma^{(t)}\right\}^{(\tau)}$ &
                        State of the entire system, {\em i.e.\/}, all
			the lattice sites comprising the system, at
			all time steps in the temporal neighborhood,
			{\em i.e.\/}, from time step $t$ to time step
			$t-\tau+1$.
			If $\tau = 1$, the superscript $(\tau)$ is
			omitted. Thus, \newline
\centerline{$\left\{\Gamma^{(t)}\right\}^{(1)} \equiv \Gamma^{(t)}$}
			\\\cline{1-1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\Phi$                & Evolution rule governing one time step
                        evolution of each lattice site as well as the
			entire system. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline
\end{tabular}%


==> chap2/TConv2.tex <==
\begin{tabular}{@{}|l|p{4in}|@{}}
\hline
Symbol & Meaning \\
\hline\hline
$\bmath{Q}$   & A vector quantity, {\em e.g.\/}, momentum.\\
$Q$           & A scalar quantity, {\em e.g.\/}, mass, energy.\\
\hline
$n$           & Number of particles.\\
$m$           & Mass.\\
$\rho$        & Density.\\
$\bmath{P}$   & Momentum.\\
$\varepsilon$ & Energy (kinetic energy).\\
$F$           & Unnormalized one particle probability distribution
		function.\\
$f$           & Normalized one particle probability distribution
		function.\\
\hline
$\bmath{Q}^{(a)}$ &
  Value of quantity $\bmath{Q}$ for particles of species $a$. \\
$\bmath{Q}_{b}^{(a)}$ &
  Value of quantity $\bmath{Q}$ for particles of species $a$ having
  velocity $\bmath{v}_{b}^{(a)}$. \\
\hline
$\bmath{Q}(\bmath{x},t)$ &
  Ensemble averaged value of quantity $\bmath{Q}$ at position
  $\bmath{x}$ at time $t$. \\
$\bmath{Q}^{(a)}(\bmath{x},t)$ &
  Ensemble averaged value of quantity $\bmath{Q}$ at position
  $\bmath{x}$ at time $t$ for particles of species $a$. \\
$\bmath{Q}_{b}^{(a)}(\bmath{x},t)$ &
  Ensemble averaged value of quantity $\bmath{Q}$ at position
  $\bmath{x}$ at time $t$ for particles of species $a$ having velocity
  $\bmath{v}_{b}^{(a)}$. \\
\hline
\end{tabular}


==> chap2/TNRRules.tex <==
\begin{tabular}{@{}|ccc|ll|@{}}
\hline
${\cal N}$ &
  ${\cal R}$ & 
    ${\cal N}^{\cal R}$ &
      Total number of evolution rules
      ($= {\cal N}^{{\cal N}^{\cal R}}$) &
        Order \\
\hline\hline
 2 & 1 & 2   & $4$                  & $[{\cal O}(10^{0})]$  \\
 2 & 2 & 4   & $16$                 & $[{\cal O}(10^{1})]$  \\
 3 & 1 & 3   & $27$                 & $[{\cal O}(10^{1})]$  \\
 4 & 1 & 4   & $256$                & $[{\cal O}(10^{2})]$  \\
 2 & 3 & 8   & $256$                & $[{\cal O}(10^{2})]$  \\
 5 & 1 & 5   & $3125$               & $[{\cal O}(10^{3})]$  \\
 3 & 2 & 9   & $19683$              & $[{\cal O}(10^{4})]$  \\
 4 & 2 & 16  & $4294967296$         & $[{\cal O}(10^{9})]$  \\
 3 & 3 & 27  & $7625597484987$      & $[{\cal O}(10^{12})]$ \\
 5 & 2 & 25  & $298023223876953125$ & $[{\cal O}(10^{17})]$ \\
 4 & 3 & 64  & $340282366920938463463374607431768211456$
				    & $[{\cal O}(10^{38})]$ \\
 5 & 3 & 125 & $2.3509887016445750159374730744444913556 \times 10^{87}$
				    & $[{\cal O}(10^{87})]$ \\
\hline
\end{tabular}


==> chap2/Tfhp.tex <==
\begin{tabular}{@{}|r|c@{~$\mapsto$~}c||r|c@{~$\mapsto$~}c|@{}}
\hline
State & \multicolumn{2}{c||}{$(\alpha_{0},\alpha_{1},\alpha_{2},
                         \alpha_{3},\alpha_{4},\alpha_{5})$ for} &
State & \multicolumn{2}{c|}{$(\alpha_{0},\alpha_{1},\alpha_{2},
                        \alpha_{3},\alpha_{4},\alpha_{5})$ for}\\
\# & Initial State & Final State &\# & Initial State & Final State \\
\hline\hline
 0 & (0,0,0,0,0,0) & (0,0,0,0,0,0) &
			32 & (1,0,0,0,0,0) & (1,0,0,0,0,0) \\
 1 & (0,0,0,0,0,1) & (0,0,0,0,0,1) &
			33 & (1,0,0,0,0,1) & (1,0,0,0,0,1) \\
 2 & (0,0,0,0,1,0) & (0,0,0,0,1,0) &
			34 & (1,0,0,0,1,0) & (1,0,0,0,1,0) \\
 3 & (0,0,0,0,1,1) & (0,0,0,0,1,1) &
			35 & (1,0,0,0,1,1) & (1,0,0,0,1,1) \\
 4 & (0,0,0,1,0,0) & (0,0,0,1,0,0) &
		    \bf 36 & (1,0,0,1,0,0) & (0,0,1,0,0,1) \\
 5 & (0,0,0,1,0,1) & (0,0,0,1,0,1) &
			& \multicolumn{1}{r@{or~}}{} & (0,1,0,0,1,0) \\
 6 & (0,0,0,1,1,0) & (0,0,0,1,1,0) &
			37 & (1,0,0,1,0,1) & (1,0,0,1,0,1) \\
 7 & (0,0,0,1,1,1) & (0,0,0,1,1,1) &
			38 & (1,0,0,1,1,0) & (1,0,0,1,1,0) \\
 8 & (0,0,1,0,0,0) & (0,0,1,0,0,0) &
			39 & (1,0,0,1,1,1) & (1,0,0,1,1,1) \\
\bf
 9 & (0,0,1,0,0,1) & (0,1,0,0,1,0) &
			40 & (1,0,1,0,0,0) & (1,0,1,0,0,0) \\
   & \multicolumn{1}{r@{or~}}{} & (1,0,0,1,0,0) &
			41 & (1,0,1,0,0,1) & (1,0,1,0,0,1) \\
10 & (0,0,1,0,1,0) & (0,0,1,0,1,0) &
		    \bf 42 & (1,0,1,0,1,0) & (0,1,0,1,0,1) \\
11 & (0,0,1,0,1,1) & (0,0,1,0,1,1) &
			43 & (1,0,1,0,1,1) & (1,0,1,0,1,1) \\
12 & (0,0,1,1,0,0) & (0,0,1,1,0,0) &
			44 & (1,0,1,1,0,0) & (1,0,1,1,0,0) \\
13 & (0,0,1,1,0,1) & (0,0,1,1,0,1) &
			45 & (1,0,1,1,0,1) & (1,0,1,1,0,1) \\
14 & (0,0,1,1,1,0) & (0,0,1,1,1,0) &
			46 & (1,0,1,1,1,0) & (1,0,1,1,1,0) \\
15 & (0,0,1,1,1,1) & (0,0,1,1,1,1) &
			47 & (1,0,1,1,1,1) & (1,0,1,1,1,1) \\
16 & (0,1,0,0,0,0) & (0,1,0,0,0,0) &
			48 & (1,1,0,0,0,0) & (1,1,0,0,0,0) \\
17 & (0,1,0,0,0,1) & (0,1,0,0,0,1) &
			49 & (1,1,0,0,0,1) & (1,1,0,0,0,1) \\
\bf
18 & (0,1,0,0,1,0) & (1,0,0,1,0,0) &
			50 & (1,1,0,0,1,0) & (1,1,0,0,1,0) \\
   & \multicolumn{1}{r@{or~}}{} & (0,0,1,0,0,1) &
			51 & (1,1,0,0,1,1) & (1,1,0,0,1,1) \\
19 & (0,1,0,0,1,1) & (0,1,0,0,1,1) &
			52 & (1,1,0,1,0,0) & (1,1,0,1,0,0) \\
20 & (0,1,0,1,0,0) & (0,1,0,1,0,0) &
			53 & (1,1,0,1,0,1) & (1,1,0,1,0,1) \\
\bf
21 & (0,1,0,1,0,1) & (1,0,1,0,1,0) &
			54 & (1,1,0,1,1,0) & (1,1,0,1,1,0) \\
22 & (0,1,0,1,1,0) & (0,1,0,1,1,0) &
			55 & (1,1,0,1,1,1) & (1,1,0,1,1,1) \\
23 & (0,1,0,1,1,1) & (0,1,0,1,1,1) &
			56 & (1,1,1,0,0,0) & (1,1,1,0,0,0) \\
24 & (0,1,1,0,0,0) & (0,1,1,0,0,0) &
			57 & (1,1,1,0,0,1) & (1,1,1,0,0,1) \\
25 & (0,1,1,0,0,1) & (0,1,1,0,0,1) &
			58 & (1,1,1,0,1,0) & (1,1,1,0,1,0) \\
26 & (0,1,1,0,1,0) & (0,1,1,0,1,0) &
			59 & (1,1,1,0,1,1) & (1,1,1,0,1,1) \\
27 & (0,1,1,0,1,1) & (0,1,1,0,1,1) &
			60 & (1,1,1,1,0,0) & (1,1,1,1,0,0) \\
28 & (0,1,1,1,0,0) & (0,1,1,1,0,0) &
			61 & (1,1,1,1,0,1) & (1,1,1,1,0,1) \\
29 & (0,1,1,1,0,1) & (0,1,1,1,0,1) &
			62 & (1,1,1,1,1,0) & (1,1,1,1,1,0) \\
30 & (0,1,1,1,1,0) & (0,1,1,1,1,0) &
			63 & (1,1,1,1,1,1) & (1,1,1,1,1,1) \\
31 & (0,1,1,1,1,1) & (0,1,1,1,1,1) &
			& \multicolumn{1}{r@{}}{} &        \\
\hline
\end{tabular}%


==> chap2/Tgencr.tex <==
\begin{tabular}{@{}|cc||ccccccc|@{}}
\hline
\multicolumn{2}{@{}|c||}{Initial States} &
\multicolumn{7}{c|@{}}{Final States ${\cal S}_{i,f}$ for $f=$} \\
\cline{3-9}
$i$
  & ${\cal S}_{i}$
    & 0 & 1 & 2 & \ldots & $f_{k}$ & \ldots & $f_{\max}-1$ \\
\hline\hline
0 & ${\cal S}_{0}$
    & ${\cal S}_{0,0}$
      & ---
	& ---
	  & \ldots
	    & ---
	      & \ldots
		& --- \\
1 & ${\cal S}_{1}$
    & ${\cal S}_{1,0}$
      & ${\cal S}_{1,1}$
	& ---
	  & \ldots
	    & ---
	      & \ldots
		& --- \\
$\vdots$
  & $\vdots$
    & $\vdots$
      & $\vdots$
        & $\vdots$
	  &
	    & $\vdots$
	      &
		& $\vdots$ \\
$k$
  & ${\cal S}_{k}$
    & ${\cal S}_{k,0}$
      & ${\cal S}_{k,1}$
        & ${\cal S}_{k,2}$
	  & \ldots
	    & ${\cal S}_{k,f_{k}}$
	      & \ldots
		& --- \\
$\vdots$
  & $\vdots$
    & $\vdots$
      & $\vdots$
        & $\vdots$
	  &
	    & $\vdots$
	      &
		& $\vdots$ \\
$n$
  & ${\cal S}_{n}$
    & ${\cal S}_{n,0}$
      & ${\cal S}_{n,1}$
        & ${\cal S}_{n,2}$
	  & \ldots
	    & ${\cal S}_{n,f_{k}}$
	      & \ldots
		& ${\cal S}_{n,f_{n}-1}$ \\
$\vdots$
  & $\vdots$
    & $\vdots$
      & $\vdots$
        & $\vdots$
	  &
	    & $\vdots$
	      &
		& $\vdots$ \\
${\cal N}_{\rm s}-1$
  & ${\cal S}_{{\cal N}_{\rm s}-1}$
    & ${\cal S}_{{\cal N}_{\rm s}-1,0}$
      & ---
	& ---
	  & \ldots
	    & ---
	      & \ldots
		& --- \\
\hline
%\multicolumn{1}{c}{$\uparrow$}
%  & \multicolumn{1}{c}{$\uparrow$}
%    & $\uparrow$
%      & $\uparrow$
%        & $\uparrow$
%	  & \ldots
%	    & $\uparrow$
%	      & \ldots
%	        & \multicolumn{1}{c}{$\uparrow$} \\
\multicolumn{1}{c}{0}
  & \multicolumn{1}{c}{1}
    & 2
      & 3
        & 4
	  & \ldots
	    & $f_{k}+2$
	      & \ldots
	        & \multicolumn{1}{c}{$f_{\max}+1$} \\
\multicolumn{9}{c}{Column Numbers}
\end{tabular}


==> chap2/Thpp2.tex <==
\begin{tabular}{@{}|r|c@{~$\mapsto$~}c||r|c@{~$\mapsto$~}c|@{}}
\hline
State &
\multicolumn{2}{c||}{$(\alpha_{0},\alpha_{1},\alpha_{2},\alpha_{3})$
for} &
State &
\multicolumn{2}{c|}{$(\alpha_{0},\alpha_{1},\alpha_{2},\alpha_{3})$
for} \\
\# & Initial State & Final State & \# & Initial State & Final State \\
\hline
\hline
    0 & (0,0,0,0) & (0,0,0,0) &      8 & (1,0,0,0) & (1,0,0,0) \\
    1 & (0,0,0,1) & (0,0,0,1) &      9 & (1,0,0,1) & (1,0,0,1) \\
    2 & (0,0,1,0) & (0,0,1,0) & \bf 10 & (1,0,1,0) & (0,1,0,1) \\
    3 & (0,0,1,1) & (0,0,1,1) &     11 & (1,0,1,1) & (1,0,1,1) \\
    4 & (0,1,0,0) & (0,1,0,0) &     12 & (1,1,0,0) & (1,1,0,0) \\
\bf 5 & (0,1,0,1) & (1,0,1,0) &     13 & (1,1,0,1) & (1,1,0,1) \\
    6 & (0,1,1,0) & (0,1,1,0) &     14 & (1,1,1,0) & (1,1,1,0) \\
    7 & (0,1,1,1) & (0,1,1,1) &     15 & (1,1,1,1) & (1,1,1,1) \\
\hline
\end{tabular}%


==> chap2/Tint1.tex <==
%\begin{tabular}{@{}|l|p{0.4\textwidth}|@{}}
\begin{tabular}{@{}|l|p{75mm}|@{}}
\hline
\multicolumn{2}{@{}|c|@{}}{Correspondence Between Elements of} \\
\hline
Cellular Automata      & Physical Systems \\
\hline\hline
Lattice of sites       & Physical position space. \\
Evolution axis         & Time axis. \\
Lattice site values    & Particles and their velocities.
                         Necessarily many (at least two) particles. \\
Evolution neighborhood & Interaction neighborhood of particles. \\
Evolution rule         & Dynamical law. \\
\hline
\end{tabular}


==> chap3/TVelOrd.tex <==
\begin{tabular}{|cc|c|c|c|}
\hline
$i$ &
  $\bmath{v}_{i}$ &
    \begin{tabular}{@{}c@{}}
      HPP gas \\
      both partitions
    \end{tabular} &
      \begin{tabular}{@{}c@{}}
	TM gas \\
	solid partition
      \end{tabular} &
	\begin{tabular}{@{}c@{}}
	  TM gas \\
	  dashed partition
	\end{tabular} \\
\hline\hline
1 & $\bmath{v}_{1}$ & $(-1,1)$  & $(-1,0)$ & $(0,1)$  \\
2 & $\bmath{v}_{2}$ & $(1,1)$   & $(0,1)$  & $(1,0)$  \\
3 & $\bmath{v}_{3}$ & $(-1,-1)$ & $(0,-1)$ & $(-1,0)$ \\
4 & $\bmath{v}_{4}$ & $(1,-1)$  & $(1,0)$  & $(0,-1)$ \\
\hline
\end{tabular}%


==> chap5/Tcinc.tex <==
\begin{tabular}{|cc|c|c@{~}l|c|}
\hline
&&\multicolumn{4}{|c|}{Contact interaction neighborhood of particles
over square spatial lattice}\\
\cline{3-6}
\# &
  \begin{tabular}{@{}c@{}}
   Discrete\\
   Velocity\\
   Set
  \end{tabular} &
    Name &
      &
        Elements &
          \begin{tabular}{@{}c@{}}
	    Number\\
	    of sites
	  \end{tabular} \\
\hline\hline
 1 & ${\cal V}_{1}$ & ${\cal L}_{1}$ &
		    & $\{
		      (0,0),
		      (\pm1,0), (0,\pm1),
		      (\pm1,\pm1),
		      (\pm2,0), (0,\pm2)
		      \}$
		    & 13 \\
 2 & ${\cal V}_{2}$ & ${\cal L}_{2}$ & ${\cal L}_{1}~\cup$
		    & $\{
		      (\pm2,\pm1), (\pm1,\pm2),
		      (\pm2,\pm2)
		      \}$
		    & 25 \\
 3 & ${\cal V}_{3}$ & ${\cal L}_{3}$ & ${\cal L}_{2}~\cup$ 
		    & $\{
		      (\pm3,0), (0,\pm3),
		      (\pm4,0), (0,\pm4)
		      \}$
		    & 33 \\
 4 & ${\cal V}_{4}$ & ${\cal L}_{4}$ & ${\cal L}_{3}~\cup$ 
		    & $\{
		      (\pm3,\pm1), (\pm1,\pm3)
		      \}$
		    & 41 \\
 5 & ${\cal V}_{5}$ & ${\cal L}_{5}$ & ${\cal L}_{4}~\cup$ 
		    & $\{
		      (\pm3,\pm2), (\pm2,\pm3),
		      (\pm3,\pm3),$
		    & 69 \\
   &                &                &
                    & $
		      (\pm4,\pm1), (\pm1,\pm4),
		      (\pm4,\pm2), (\pm2,\pm4)
		      \}$
		    & \\
\hline
\end{tabular}


==> chap5/Trprime.tex <==
\begin{tabular}{|cc|c|cc|c|}
\hline
\# &
  \begin{tabular}{@{}c@{}}
    Discrete\\
    Velocity\\
    Set
  \end{tabular} &
    $4|\bmath{r}'|^{2}$ &
      \begin{tabular}{@{}c@{}}
	Number of \\
	lattice sites\\
        in contact\\
	interaction\\
	neighborhood
      \end{tabular} &
	\begin{tabular}{@{}c@{}}
	  Number of \\
	  lattice sites in\\
	  smallest field\\
	  interaction\\
	  neighborhood
	\end{tabular} &
	  \begin{tabular}{@{}c@{}}
	    Maximum value \\
	    of $4\tilde{R}_{\rm I}^{2}$ for \\
	    smallest field\\
	    interaction\\
	    neighborhood
	  \end{tabular} \\
\hline\hline
 1 & ${\cal V}_{1}$ &  9 & 13 & 13 & 10 \\
 2 & ${\cal V}_{2}$ & 18 & 25 & 25 & 25 \\
 3 & ${\cal V}_{3}$ & 49 & 33 & 49 & 50 \\
 4 & ${\cal V}_{4}$ & 49 & 41 & 49 & 50 \\
 5 & ${\cal V}_{5}$ & 58 & 69 & 69 & 74 \\
\hline
\end{tabular}


==> chap5/Tscin.tex <==
\begin{tabular}{|cc|ccc|r@{~}l|}
\hline
  $i$ &
    ${\cal V}$ &
      ${\cal N}_{\rm v}$ &
        ${\cal N}_{\rm s}$ &
	  ${\cal N}_{{\cal L}_{\rm C}}$ &
	    \multicolumn{2}{|c|}{\rule{0pt}{12pt}%
	    $\left({\cal N}_{\rm s}\right)^{{\cal N}_{{\cal
	    L}_{\rm C}}} = {\cal N}_{\rm s,cin}$} \\
\hline
\hline
1 & ${\cal V}_{1}$ & 4& 5&13& $ 5^{13}$&$\approx1.22\times10^{9} $
\rule{0pt}{11pt} \\
2 & ${\cal V}_{2}$ & 8& 9&25& $ 9^{25}$&$\approx7.18\times10^{23}$ \\
3 & ${\cal V}_{3}$ & 8& 9&33& $ 9^{33}$&$\approx3.09\times10^{31}$ \\
4 & ${\cal V}_{4}$ &12&13&41& $13^{41}$&$\approx4.70\times10^{45}$ \\
5 & ${\cal V}_{5}$ &20&21&69& $21^{69}$&$\approx1.71\times10^{91}$ \\
\hline
\end{tabular}%



==> chap5/Ttfin.tex <==
\begin{tabular}{|cc|clll|c|}
\hline
\multicolumn{2}{|c|}{Range of $\displaystyle4\tilde{R}_{\rm I}^{2}$}
    & \multicolumn{4}{c|}{Coordinates of lattice sites lying in}
      & Number \\
$\displaystyle4\tilde{R}_{\rm I_{min}}^{2}$
  & $\displaystyle4\tilde{R}_{\rm I_{max}}^{2}$
    & \multicolumn{4}{c|}{the field interaction neighborhood}
      & of sites \\
\hline\hline
 0 &  1 &          & $(0,0)$        &                & &  1 \\
 1 &  2 & $\oplus$ & $(\pm1,0)$,    & $(0,\pm1)$     & &  5 \\
 2 &  9 & $\oplus$ & $(\pm1,\pm1)$  &                & &  9 \\
 9 & 10 & $\oplus$ & $(\pm2,0)$,    & $(0,\pm2)$     & & 13 \\
10 & 18 & $\oplus$ & $(\pm2,\pm1)$, & $(\pm1,\pm2)$  & & 21 \\
18 & 25 & $\oplus$ & $(\pm2,\pm2)$  &                & & 25 \\
25 & 26 & $\oplus$ & $(\pm3,0)$,    & $(0,\pm3)$     & & 29 \\
26 & 34 & $\oplus$ & $(\pm3,\pm1)$, & $(\pm1,\pm3)$  & & 37 \\
34 & 49 & $\oplus$ & $(\pm3,\pm2)$, & $(\pm2,\pm3)$  & & 45 \\
49 & 50 & $\oplus$ & $(\pm4,0)$,    & $(0,\pm4)$     & & 49 \\
50 & 58 & $\oplus$ & $(\pm4,\pm1)$, & $(\pm1,\pm4)$,
                                    & $(\pm3,\pm3)$    & 61 \\
58 & 74 & $\oplus$ & $(\pm4,\pm2)$, & $(\pm2,\pm4)$  & & 69 \\
74 & 81 & $\oplus$ & $(\pm4,\pm3)$, & $(\pm3,\pm4)$  & & 77 \\
\hline
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 0& 1 ~ $1/2$         & & $(0,0)$        &                &  &  1 \\
% 1& 2 ~ $1/\sqrt{2}$  &+& $(\pm1,0)$,    & $(0,\pm1)$     &  &  5 \\
% 2& 9 ~ $3/2$         &+& $(\pm1,\pm1)$  &                &  &  9 \\
% 9&10 ~ $\sqrt{5/2}$  &+& $(\pm2,0)$,    & $(0,\pm2)$     &  & 13 \\
%10&18 ~ $3/\sqrt{2}$  &+& $(\pm2,\pm1)$, & $(\pm1,\pm2)$  &  & 21 \\
%18&25 ~ $5/2$         &+& $(\pm2,\pm2)$  &                &  & 25 \\
%25&26 ~ $\sqrt{13/2}$ &+& $(\pm3,0)$,    & $(0,\pm3)$     &  & 29 \\
%26&34 ~ $\sqrt{17/2}$ &+& $(\pm3,\pm1)$, & $(\pm1,\pm3)$  &  & 37 \\
%34&49 ~ $7/2$         &+& $(\pm3,\pm2)$, & $(\pm2,\pm3)$  &  & 45 \\
%49&50 ~ $5/\sqrt{2}$  &+& $(\pm4,0)$,    & $(0,\pm4)$     &  & 49 \\
%50&58 ~ $\sqrt{29/2}$ &+& $(\pm4,\pm1)$, & $(\pm1,\pm4)$, &
%                          $(\pm3,\pm3)$                      & 61 \\
%58&74 ~ $\sqrt{37/2}$ &+& $(\pm4,\pm2)$, & $(\pm2,\pm4)$  &  & 69 \\
%74&81 ~ $9/2$         &+& $(\pm4,\pm3)$, & $(\pm3,\pm4)$  &  & 77 \\


==> chap5/Tvsets.tex <==
\begin{tabular}{|cc|c@{~}l|c|}
\hline
\multicolumn{5}{|c|}{Some discrete velocity sets over square spatial
lattice}\\
\hline
\# & Name & & Elements & Number of elements \\
\hline\hline
 1 & ${\cal V}_{1}$ &                     &
                      $\{(\pm1,0),(0,\pm1)\}$       & 4 \\
 2 & ${\cal V}_{2}$ & ${\cal V}_{1}~\cup$ &
                      $\{(\pm1,\pm1)\}$             & 8 \\
 3 & ${\cal V}_{3}$ & ${\cal V}_{1}~\cup$ &
                      $\{(\pm2,0),(0,\pm2)\}$       & 8 \\
 4 & ${\cal V}_{4}$ & ${\cal V}_{2}~\cup$ &
                      $\{(\pm2,0),(0,\pm2)\}$       & 12 \\
 5 & ${\cal V}_{5}$ & ${\cal V}_{4}~\cup$ &
                      $\{(\pm2,\pm1),(\pm1,\pm2)\}$ & 20 \\
\hline
\end{tabular}


==> chap6/TSPLG1BCCProbs.tex <==
\begin{tabular}{@{}|c|cll|@{}}
\hline
  \begin{tabular}{@{}c@{}}
    BCC \# \\
     $i$
  \end{tabular} &
    ${\cal N}_{\rm iso}^{(i)}$ &
      $\hat{P}^{(i)}$ &
        $P^{(i)} = {\cal N}_{\rm iso}^{(i)} \hat{P}^{(i)}$ \\
\hline\hline
  1
    & 2
      & $(n/4)^{2}$
	& $2(n/4)^{2}$ \\
  2
    & 2
      & $(n/4)^{2}(1-n/4)(1-3n/4+n^{2}/4)$
	& $2(n/4)^{2}(1-n/4)(1-3n/4+n^{2}/4)$ \\
  3
    & 4
      & $(n/4)^{2}(1-n/4)(1-3n/4+n^{2}/4)$
	& $4(n/4)^{2}(1-n/4)(1-3n/4+n^{2}/4)$ \\
  4
    & 4
      & $(n/4)^{3}(1-n/2)^{2}$
	& $4(n/4)^{3}(1-n/2)^{2}$ \\
  5
    & 1
      & $(n/4)^{4}(1-n)$
	& $(n/4)^{4}(1-n)$ \\
\hline
\end{tabular}%


==> chap7/Tprob.tex <==
\begin{tabular}{|c|lrr|}
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
BCC & \multicolumn{3}{c|}{Probability of occurrence of BCCs
			  including all isometries
			  for mean particle density of} \\
\#  & \multicolumn{1}{c}{$n$}
    & \multicolumn{1}{c}{$n=0.05$}
    & \multicolumn{1}{c|}{$n=0.10$} \\
\hline\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
1   & $2(n/4)^{2}$
    & $3.125\times10^{-4}$
    & $1.25\times10^{-3}$           \\
2   & $2(n/4)^{2}(1-n/4)(1-3n/4+n^{2}/4)$
    & $2.9721435546875\times10^{-4}$
    & $1.130390625\times10^{-3}$        \\
3   & $4(n/4)^{2}(1-n/4)(1-3n/4+n^{2}/4)$
    & $5.944287109375\times10^{-4}$
    & $2.26078125\times10^{-3}$         \\
4   & $4(n/4)^{3}(1-n/2)^{2}$
    & $7.4267578125\times10^{-6}$
    & $5.640625\times10^{-5}$        \\
5   & $(n/4)^{4}(1-n)$
    & $2.3193359375\times10^{-8}$
    & $3.515625\times10^{-7}$     \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}%


==> chap7/Tstpff.tex <==
{\tabcolsep1mm\begin{tabular}{|l|c|cccccccc|}
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      & FCC & \multicolumn{8}{c|}{Solutions} \\%\cline{2-9}
      & \#  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
\hline\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      & (1) & 1 & 1 & 1 & - & - & - & - & - \\
STP   & (2) & 1 & 1 & 1 & - & - & - & - & - \\
Set-1 & (3) & 1 & - & - & - & - & - & - & - \\
      & (4) & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
      & (5) & 1 & 1 & 1 & 1 & 1 & 1 & 1 & - \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      & (1) & 1 & 1 & 1 & - & - & - & - & - \\
STP   & (2) & 1 & 1 & 1 & - & - & - & - & - \\
Set-2 & (3) & 1 & - & - & - & - & - & - & - \\
      & (4) & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
      & (5) & 0 & 0 & 0 & 0 & 0 & 0 & 1 & - \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      & (1) & 1 & 1 & 1 & - & - & - & - & - \\
STP   & (2) & 1 & 1 & 1 & - & - & - & - & - \\
Set-3 & (3) & 1 & - & - & - & - & - & - & - \\
      & (4) & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
      & (5) & 1 & 1 & 1 & 1 & 1 & 1 & 1 & - \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      & (1) & 1 & 1 & 1 & - & - & - & - & - \\
STP   & (2) & 1 & 1 & 1 & - & - & - & - & - \\
Set-4 & (3) & 1 & - & - & - & - & - & - & - \\
      & (4) & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
      & (5) & 0 & 0 & 0 & 0 & 0 & 0 & 1 & - \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      & (1) & 1 & 1 & 1 & - & - & - & - & - \\
STP   & (2) & 1 & 1 & 1 & - & - & - & - & - \\
Set-5 & (3) & 1 & - & - & - & - & - & - & - \\
      & (4) & 1 & 1 & 1 & 1 & 1 & 0 & 0 & 0 \\
      & (5) & 1 & 1 & 1 & 1 & 1 & 1 & 1 & - \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}}%


==> chap7/Tstpfw.tex <==
\begin{tabular}{|c|ccc|}
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FCC & \multicolumn{3}{c|}{Solutions}\\
\#  & (1) & (2) & (3) \\
\hline\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(1) & 1 & 1 & 1 \\
(2) & 1 & 1 & 1 \\
(3) & 1 & 1 & 1 \\
(4) & 1 & 1 & - \\
(5) & 1 & 1 & - \\
(6) & 1 & 1 & - \\
(7) & 1 & 1 & - \\
(8) & 1 & - & - \\
(9) & 1 & - & - \\
\hline%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}%


==> chap7/Tvacfit.tex <==
\begin{tabular}{|c|c|ccrrc|}
\hline
$n$ &
  \begin{tabular}{@{}c@{}}
    STP\\
    set\\
  \end{tabular}&
    $t_{1}$ &
      $t_{2}$ &
	\multicolumn{1}{c}{$b$} &
	  \multicolumn{1}{c}{$\alpha$} &
	    \begin{tabular}{@{}c@{}}
	      Sum of square\\
	      residuals\\
	    \end{tabular}\\\hline\hline
     & 1
       & 20
	 & 450
	   & $0.103017(\pm0.00834741)$
	     & $0.977219(\pm0.0206897)$
	       & $6.26323\times10^{-5}$ \\
     & 2
       & 20
	 & 450
	   & $0.123940(\pm0.00986215)$
	     & $1.024910(\pm0.0206068)$
	       & $5.80601\times10^{-5}$ \\
0.05 & 3
       & 20
	 & 450
	   & $0.109639(\pm0.00891527)$
	     & $0.990357(\pm0.0208452)$
	       & $6.38264\times10^{-5}$ \\
     & 4
       & 20
	 & 450
	   & $0.112269(\pm0.00897831)$
	     & $0.992581(\pm0.0205145)$
	       & $6.35078\times10^{-5}$ \\
     & 5
       & 20
	 & 450
	   & $0.114008(\pm0.00996523)$
	     & $1.005730(\pm0.0225099)$
	       & $6.98894\times10^{-5}$ \\
\hline
     & 1
       & 15
	 & 450
	   & $0.1653850(\pm0.00857383)$
	     & $1.064610(\pm0.0145795)$
	       & $5.63381\times10^{-5}$ \\
     & 2
       & 15
	 & 450
	   & $0.1460890(\pm0.00695378)$
	     & $1.031970(\pm0.0132400)$
	       & $4.83276\times10^{-5}$ \\
0.10 & 3
       & 15
	 & 450
	   & $0.0986275(\pm0.00391530)$
	     & $0.877855(\pm0.0104187)$
	       & $5.36523\times10^{-5}$ \\
     & 4
       & 15
	 & 450
	   & $0.1020970(\pm0.00408149)$
	     & $0.887570(\pm0.0105332)$
	       & $5.38821\times10^{-5}$ \\
     & 5
       & 15
	 & 450
	   & $0.1619370(\pm0.00829087)$
	     & $1.054900(\pm0.0143522)$
	       & $5.70097\times10^{-5}$ \\
\hline
\end{tabular}


==> chap8/Tshkvelc.tex <==
\begin{tabular}{|l|cc|}
\hline
\begin{tabular}{@{}c@{}}
  Position\\
  relative\\
  to peak\\
  of shock\\
\end{tabular} &
  $f$ &
    \begin{tabular}{@{}c@{}}
      Velocity in the\\
      time interval\\
      $[120,490]$\\
    \end{tabular} \\
\hline\hline
      & $0.5$ & $0.804051 (\pm2.73304\times10^{-3})$ \\
      & $0.6$ & $0.815798 (\pm2.55853\times10^{-3})$ \\
Left  & $0.7$ & $0.833323 (\pm2.95727\times10^{-3})$ \\
      & $0.8$ & $0.851996 (\pm3.57283\times10^{-3})$ \\
      & $0.9$ & $0.871771 (\pm4.34943\times10^{-3})$ \\\hline
Peak  & $1.0$ & $0.901751 (\pm3.46226\times10^{-3})$ \\\hline
      & $0.9$ & $0.882482 (\pm2.98834\times10^{-3})$ \\
      & $0.8$ & $0.877436 (\pm2.70390\times10^{-3})$ \\
Right & $0.7$ & $0.876289 (\pm2.41452\times10^{-3})$ \\
      & $0.6$ & $0.878140 (\pm2.08874\times10^{-3})$ \\
      & $0.5$ & $0.885965 (\pm2.04651\times10^{-3})$ \\
\hline
\end{tabular}%
\comment{

These values are in the order vl5...vl9 vc vr9...vr5
The variation in 68.3% confidance interval has been multiplied by 1000.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		      Incorrect old calculations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

90 <= t <= 520
--------------
      & $0.5$ & $1.22335 (\pm9.21882)$ \\
      & $0.6$ & $1.20605 (\pm9.60299)$ \\
Left  & $0.7$ & $1.18681 (\pm8.78703)$ \\
      & $0.8$ & $1.16640 (\pm6.44415)$ \\
      & $0.9$ & $1.14295 (\pm6.02491)$ \\\hline
Peak  & $1.0$ & $1.11660 (\pm3.77353)$ \\\hline
      & $0.9$ & $1.13278 (\pm5.60682)$ \\
      & $0.8$ & $1.13143 (\pm6.75396)$ \\
Right & $0.7$ & $1.13355 (\pm5.29502)$ \\
      & $0.6$ & $1.12743 (\pm5.23285)$ \\
      & $0.5$ & $1.12478 (\pm3.17897)$ \\\hline

100 <= t <= 510
---------------
      & $0.5$ & $1.22243 (\pm9.53862)$ \\
      & $0.6$ & $1.21058 (\pm8.73089)$ \\
Left  & $0.7$ & $1.19675 (\pm5.68985)$ \\
      & $0.8$ & $1.17272 (\pm5.03101)$ \\
      & $0.9$ & $1.14665 (\pm5.23556)$ \\\hline
Peak  & $1.0$ & $1.11658 (\pm4.06867)$ \\\hline
      & $0.9$ & $1.13973 (\pm3.66173)$ \\
      & $0.8$ & $1.14106 (\pm3.71919)$ \\
Right & $0.7$ & $1.13953 (\pm3.79325)$ \\
      & $0.6$ & $1.12922 (\pm5.30722)$ \\
      & $0.5$ & $1.12378 (\pm3.43089)$ \\\hline

120 <= t <= 500
--------------
      & $0.5$ & $1.24528 (\pm4.11419)$ \\
      & $0.6$ & $1.22763 (\pm3.80110)$ \\
Left  & $0.7$ & $1.20249 (\pm4.29305)$ \\
      & $0.8$ & $1.17660 (\pm4.97245)$ \\
      & $0.9$ & $1.14895 (\pm5.54002)$ \\\hline
Peak  & $1.0$ & $1.11082 (\pm4.18527)$ \\\hline
      & $0.9$ & $1.13531 (\pm3.84938)$ \\
      & $0.8$ & $1.14083 (\pm3.39704)$ \\
Right & $0.7$ & $1.14123 (\pm2.98246)$ \\
      & $0.6$ & $1.13565 (\pm3.07242)$ \\
      & $0.5$ & $1.12622 (\pm2.81954)$ \\\hline

120 <= t <= 490
--------------
      & $0.5$ & $1.24370 (\pm4.22323)$ \\
      & $0.6$ & $1.22579 (\pm3.84052)$ \\
Left  & $0.7$ & $1.20002 (\pm4.25433)$ \\
      & $0.8$ & $1.17371 (\pm4.91703)$ \\
      & $0.9$ & $1.14709 (\pm5.71734)$ \\\hline
Peak  & $1.0$ & $1.10895 (\pm4.25355)$ \\\hline
      & $0.9$ & $1.13317 (\pm3.83339)$ \\
      & $0.8$ & $1.13968 (\pm3.50854)$ \\
Right & $0.7$ & $1.14118 (\pm3.14125)$ \\
      & $0.6$ & $1.13877 (\pm2.70597)$ \\
      & $0.5$ & $1.12871 (\pm2.60463)$ \\\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		      Correct new calculations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

120 <= t <= 490
--------------
      & $0.5$ & $0.804051 (\pm2.73304)$ \\
      & $0.6$ & $0.815798 (\pm2.55853)$ \\
Left  & $0.7$ & $0.833323 (\pm2.95727)$ \\
      & $0.8$ & $0.851996 (\pm3.57283)$ \\
      & $0.9$ & $0.871771 (\pm4.34943)$ \\\hline
Peak  & $1.0$ & $0.901751 (\pm3.46226)$ \\\hline
      & $0.9$ & $0.882482 (\pm2.98834)$ \\
      & $0.8$ & $0.877436 (\pm2.70390)$ \\
Right & $0.7$ & $0.876289 (\pm2.41452)$ \\
      & $0.6$ & $0.878140 (\pm2.08874)$ \\
      & $0.5$ & $0.885965 (\pm2.04651)$ \\\hline

}


==> chap8/Tshkvelr.tex <==
\begin{tabular}{|l|cccc|}
\hline
\begin{tabular}{@{}c@{}}
  Position\\
  relative\\
  to peak\\
  of shock\\
\end{tabular} &
  $f$ &
    $t_{1}$ &
      $t_{2}$ &
	\begin{tabular}{@{}c@{}}
	  Velocity in the\\
	  time interval\\
	  $[t_{1},t_{2}]$\\
	\end{tabular} \\
\hline\hline
      & $0.5$ & $520$ & $560$ & $2.44485 (\pm0.1658080)$ \\
      & $0.6$ & $520$ & $550$ & $2.97814 (\pm0.1455680)$ \\
Left  & $0.7$ & $520$ & $540$ & $3.85541 (\pm0.0835339)$ \\
      & $0.8$ & $520$ & $540$ & $4.15020 (\pm0.0166841)$ \\
      & $0.9$ & $520$ & $540$ & $4.67519 (\pm0.7981170)$ \\\hline
Peak  & $1.0$ & $520$ & $530$ & $5.30000 (\pm0.7502830)$ \\\hline
      & $0.9$ & $510$ & $530$ & $2.37101 (\pm0.2407780)$ \\
      & $0.8$ & $500$ & $520$ & $2.33623 (\pm0.1694610)$ \\
Right & $0.7$ & $490$ & $520$ & $1.61750 (\pm0.0846657)$ \\
      & $0.6$ & $490$ & $510$ & $1.96068 (\pm0.0838737)$ \\
      & $0.5$ & $490$ & $510$ & $1.35062 (\pm0.0166910)$ \\
\hline
\end{tabular}%

